Using ConceptNet to Teach Common Sense to an Automated Theorem Prover

The CoRg system is a system to solve commonsense reasoning problems. The core of the CoRg system is the automated theorem prover Hyper that is fed with large amounts of background knowledge. This background knowledge plays a crucial role in solving commonsense reasoning problems. In this paper we present different ways to use knowledge graphs as background knowledge and discuss challenges that arise.

==> eptcsdata.tex <==
\providecommand{\firstpage}{19}
\providecommand{\publicationstatus}{M. Suda, S. Winkler (Eds.): Second International Workshop\\
on Automated Reasoning: Challenges, Applications,\\
Directions, Exemplary Achievements (ARCADE 2019)\\
EPTCS 311, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.311.3}{10.4204/EPTCS.311.3}}
\pdfoutput=1

